Pure Tensor Program Rewriting via Access Patterns (Representation Pearl)

Tensor kernels in machine learning (ML) often correspond to pure mathematical expressions, making term rewriting an attractive strategy for optimization and mapping to specialized hardware accelerators. However, existing ML intermediate representations (IRs) tend to either be \textit{pure but high-level}, making low-level rewrites to hardware targets inexpressible, or \textit{low-level but impure}, hampering the use of term rewriting altogether. This paper introduces Glenside, a pure IR whose core abstraction -- the \textit{access pattern} -- enables low-level, layout-aware, hardware-centric program rewrites. We demonstrate how term rewriting in Glenside can be used to map program fragments to hardware accelerator invocations and automatically discover classic data layout transformations like \texttt{im2col}. Glenside establishes a new foundation for exploring further term rewriting techniques in optimizing low-level tensor programs.

==> 2021-01-28-old-intro.tex <==
\section{Introduction}

The explosive growth
  of deep learning
  over the past decade
  has reinvigorated the field
  of computer architecture.
 The need for powerful
  custom-built
  deep learning
  accelerators
  has given architects
  a new target.
\textit{Some sentences
  explaining
  why we need
  automated 
  softare-hardware codesign.}
Yet
  designing an accelerator
  for a workload
  remains
  a mostly manual task
  for hardware and compiler engineers.
  
From the workload's perspective,
  accelerators are not complicated:
  tensors with specific memory layouts
  (e.g. \texttt{NCHW})
  flow out of memory,
  through a collection of hardware modules,
  and back to memory.
Each operator in the program
  is either
  computed by a module
  on the accelerator,
  or it must be computed on the host.
Each module
  has specific data layout expectations
  which must be fulfilled
  for computation to be correct.
Operators
  can be covered in numerous ways
  by the hardware.
For example,
  weight-stationary systolic arrays
  can compute convolutions
  in \texttt{conv2d} mode---%
  by applying filters
  over a sliding window
  of an image---%
  or the activations can be transformed
  into \texttt{im2col} format
  and the systolic array can operate
  in standard
  matrix-multiplication
  (also called ``fully connected" or \texttt{fc})
  mode.
  
Deep learning compiler frameworks,
  e.g.~TVM\cite{tvm},
  are designed around optimizing
  for \textit{existing} hardware:
  CPUs, GPUs,
  and increasingly,
  custom hardware accelerators
  such as VTA\cite{vta} or \textit{other examples}.
These frameworks
  take the hardware target
  as a given,
  and explore a range 
  of software optimizations
  for the hardware target.
These optimizations include
  operator fusion,
  in which operators
  can be intelligently chained
  without needing to write intermediate data
  to memory,
  and \textit{other examples}.
The development
  of software optimizations
  is driven by existing hardware,
  and the feedback loop
  for improving software
  is instantaneous:
  software engineers
  can simply recompile their workloads
  and run them on the hardware
  to determine speedup.
However, 
  the same is not the case
  for improving hardware.
The feedback loop
  for improving hardware
  is much longer;
  hardware synthesis
  and hardware simulation
  are much slower
  than software compilation
  and software execution.
% Hm...I feel like this isn't
% actually sending the message
% I want to send.
Additionally,
  changes to the hardware
  may result in 
  nontrivial changes 
  in the software.

With the growing popularity
  of reprogrammable hardware
  such as FPGAs and CGRAs,
  the assumption that hardware
  must be a fixed target
  will soon be invalid.
In fact,
  some have argued
  that this view of hardware
  has put us in a rut;
  as long as we continue
  to optimize for 
  a select few hardware platforms
  we will restrict the diversity
  of software workloads 
  \textit{cite hardware lotto;
  make sure 
  this is 
  what they actually say}.
This work
  details
As a field,
  we must consciously take steps
  to avoid getting stuck in this rut.
We need to encourage
  and enable
  the development of
  new hardware architectures.
We need to avoid
  digging ourselves deeper
  into the rut
  than we already are.
We must avoid
  giving in further
  to the confirmation bias
  that our current architectures
  are truly the best architectures.
\texttt{/rant}
Viewing hardware
  as just one more aspect
  of the overall program
  opens an even wider space
  of potential optimizations.

To this end,
  we designed \g{},
  a program representation
  which captures both hardware
  and software
  concerns
  simultaneously.
Rather than make assumptions
  about the underlying hardware,
  \g{}
  reifies some hardware concepts
  (such as hardware modules
    and memory residency)
  in the representation itself.

\g{}
  is specifically designed
  as a language to be used
  in equality graphs \cite{egraph stuff}.
\textit{Equality graphs,}
  or \textit{egraphs},
  are a data structure
  designed to represent
  a massive search space
  of equivalent programs.

The contributions
  of this work are:
\begin{itemize}
\item \g{}, a language...
\item
  A set of rewrites over \g{},
  and a procedure for applying them,
  which enables a massive
  design space exploration
  from a single program.
\item
  A methodology
  for thinking about 
  \hwsw{} codesign
  as a compilation problem.
\end{itemize}

==> submissions/2021-01-28-old-intro.tex <==
\section{Introduction}

The explosive growth
  of deep learning
  over the past decade
  has reinvigorated the field
  of computer architecture.
 The need for powerful
  custom-built
  deep learning
  accelerators
  has given architects
  a new target.
\textit{Some sentences
  explaining
  why we need
  automated 
  softare-hardware codesign.}
Yet
  designing an accelerator
  for a workload
  remains
  a mostly manual task
  for hardware and compiler engineers.
  
From the workload's perspective,
  accelerators are not complicated:
  tensors with specific memory layouts
  (e.g. \texttt{NCHW})
  flow out of memory,
  through a collection of hardware modules,
  and back to memory.
Each operator in the program
  is either
  computed by a module
  on the accelerator,
  or it must be computed on the host.
Each module
  has specific data layout expectations
  which must be fulfilled
  for computation to be correct.
Operators
  can be covered in numerous ways
  by the hardware.
For example,
  weight-stationary systolic arrays
  can compute convolutions
  in \texttt{conv2d} mode---%
  by applying filters
  over a sliding window
  of an image---%
  or the activations can be transformed
  into \texttt{im2col} format
  and the systolic array can operate
  in standard
  matrix-multiplication
  (also called ``fully connected" or \texttt{fc})
  mode.
  
Deep learning compiler frameworks,
  e.g.~TVM\cite{tvm},
  are designed around optimizing
  for \textit{existing} hardware:
  CPUs, GPUs,
  and increasingly,
  custom hardware accelerators
  such as VTA\cite{vta} or \textit{other examples}.
These frameworks
  take the hardware target
  as a given,
  and explore a range 
  of software optimizations
  for the hardware target.
These optimizations include
  operator fusion,
  in which operators
  can be intelligently chained
  without needing to write intermediate data
  to memory,
  and \textit{other examples}.
The development
  of software optimizations
  is driven by existing hardware,
  and the feedback loop
  for improving software
  is instantaneous:
  software engineers
  can simply recompile their workloads
  and run them on the hardware
  to determine speedup.
However, 
  the same is not the case
  for improving hardware.
The feedback loop
  for improving hardware
  is much longer;
  hardware synthesis
  and hardware simulation
  are much slower
  than software compilation
  and software execution.
% Hm...I feel like this isn't
% actually sending the message
% I want to send.
Additionally,
  changes to the hardware
  may result in 
  nontrivial changes 
  in the software.

With the growing popularity
  of reprogrammable hardware
  such as FPGAs and CGRAs,
  the assumption that hardware
  must be a fixed target
  will soon be invalid.
In fact,
  some have argued
  that this view of hardware
  has put us in a rut;
  as long as we continue
  to optimize for 
  a select few hardware platforms
  we will restrict the diversity
  of software workloads 
  \textit{cite hardware lotto;
  make sure 
  this is 
  what they actually say}.
This work
  details
As a field,
  we must consciously take steps
  to avoid getting stuck in this rut.
We need to encourage
  and enable
  the development of
  new hardware architectures.
We need to avoid
  digging ourselves deeper
  into the rut
  than we already are.
We must avoid
  giving in further
  to the confirmation bias
  that our current architectures
  are truly the best architectures.
\texttt{/rant}
Viewing hardware
  as just one more aspect
  of the overall program
  opens an even wider space
  of potential optimizations.

To this end,
  we designed \g{},
  a program representation
  which captures both hardware
  and software
  concerns
  simultaneously.
Rather than make assumptions
  about the underlying hardware,
  \g{}
  reifies some hardware concepts
  (such as hardware modules
    and memory residency)
  in the representation itself.

\g{}
  is specifically designed
  as a language to be used
  in equality graphs \cite{egraph stuff}.
\textit{Equality graphs,}
  or \textit{egraphs},
  are a data structure
  designed to represent
  a massive search space
  of equivalent programs.

The contributions
  of this work are:
\begin{itemize}
\item \g{}, a language...
\item
  A set of rewrites over \g{},
  and a procedure for applying them,
  which enables a massive
  design space exploration
  from a single program.
\item
  A methodology
  for thinking about 
  \hwsw{} codesign
  as a compilation problem.
\end{itemize}
